HeteroEdge: Addressing Asymmetry in Heterogeneous Collaborative Autonomous Systems

Gathering knowledge about surroundings and generating situational awareness for IoT devices is of utmost importance for systems developed for smart urban and uncontested environments. For example, a large-area surveillance system is typically equipped with multi-modal sensors such as cameras and LIDARs and is required to execute deep learning algorithms for action, face, behavior, and object recognition. However, these systems face power and memory constraints due to their ubiquitous nature, making it crucial to optimize data processing, deep learning algorithm input, and model inference communication. In this paper, we propose a self-adaptive optimization framework for a testbed comprising two Unmanned Ground Vehicles (UGVs) and two NVIDIA Jetson devices. This framework efficiently manages multiple tasks (storage, processing, computation, transmission, inference) on heterogeneous nodes concurrently. It involves compressing and masking input image frames, identifying similar frames, and profiling devices to obtain boundary conditions for optimization.. Finally, we propose and optimize a novel parameter split-ratio, which indicates the proportion of the data required to be offloaded to another device while considering the networking bandwidth, busy factor, memory (CPU, GPU, RAM), and power constraints of the devices in the testbed. Our evaluations captured while executing multiple tasks (e.g., PoseNet, SegNet, ImageNet, DetectNet, DepthNet) simultaneously, reveal that executing 70% (split-ratio=70%) of the data on the auxiliary node minimizes the offloading latency by approx. 33% (18.7 ms/image to 12.5 ms/image) and the total operation time by approx. 47% (69.32s to 36.43s) compared to the baseline configuration (executing on the primary node).

==> sections/Applications.tex <==
% % \section{\textbf{Applications \& Requirements}}
% % \subsection{Scenario}
% % There are current issues surrounding military recruitment rates in the United States of America. A large portion of American youth is not fit to be recruited into military branches. One major health issue that eliminates much of the youth from being recruited is obesity, but other health issues also prevent many individuals from qualifying to be enlisted. Additionally, the COVID-19 Pandemic which began in the year 2020 has further discouraged people to enlist and made the job of recruiters increasingly difficult \cite{Covid19}. Military resources decrease immensely due to cultural health and socio-economical changes. However, by optimizing wireless sensor networks to run multiple deep learning algorithms concurrently with seamless rendering and low inference latency, we can address this problem.\\
% % \begin{figure}[htbp]
% %     % \vspace{-3ex}
% %     \centering
% %     \includegraphics[width=0.4\textwidth]{sections/Images/scanario.jpg}
% %     \hfill
% %     \caption{Enemy base information using object detection and jungle environment.}
% %     \label{fig:scanario}
% %     \vspace{-2ex}
% % \end{figure}
% % \\
% % In a military mission, sensors can be placed on the ground or mounted on unmanned aerial vehicles(UAVs) and unmanned ground vehicles (UGVs) to acquire information. In order to locate bounding boxes where the targets can be found, Object detection algorithms will be used to analyze the sensory data that has been obtained. Fast and accurate object detectors can increase the lethality and survivability of the weapon platform/soldiers.\\
% % Apart from enemy position or detection, Army needs to find a suitable way in a jungle/forest to pass their weapons, trucks, and other vehicles.UAV and UGV help to find a path using sensor data in a jungle environment. Whether the tactical situation involves the invasion of a variety of combat vehicles entering the specific forest path.\\
% % The wireless sensor network may contain multiple unmanned ground vehicles, UGVs, and unmanned aerial
% % vehicles, or UAVs or drones. These devices may be positioned in multiple locations to monitor the area and provide further intelligence and surveillance for the military. They may detect suspicious activity, detect identities of people in the area for security purposes, or manage other safety precautions. Soldiers
% % may be deployed where they are most needed if they are replaced by these devices.


% \section{\textbf{\name Profiling Engine}}
% \label{sec:profiling}


% \textbf{Implementation. }
% The publisher-subscriber architecture \cite{publisher_subcriber} is a messaging pattern that lets different nodes in a distributed system communicate with each other. Nodes in this architecture can either be a publisher or a subscriber. Publishers create data and send it to a central message broker. The central message broker then sends the data to subscribers who have asked for it.
% In this research, we used the MQTT (Message Queuing Telemetry Transport)\cite{MQTT} protocol. MQTT is based on the publish-subscribe pattern and is designed to be lightweight.\\
% When offloading images over MQTT over Wi-Fi, the latency is determined by various factors, including image size, available bandwidth, and the computing capability of the devices involved.
% Larger images, in general, take longer to transmit and have more latency. The Wi-Fi network's available bandwidth will also impact latency, as a congested network may result in longer transmission times.
% The processing power of the offloading devices will also have an impact on latency, as more powerful devices will be able to process the photos faster.
% We investigated with multiple wifi frequency bands, 2.4 Ghz and 5 Ghz, offloading different sizes of photos and recording latency for them; Fig. \ref{fig:mqtt_latency}(a) depicts the results.
% % \begin{figure}[htbp]
% %     % \vspace{-5ex}
% %     \centering
% %     \includegraphics[width=.20\textwidth]{sections/Images/Mqtt_latency.png}
% %     \hfill
% %     \caption{For different network bands \& different sizes of images latency for MQTT protocol are different. It will change with the size of the images }
% %     \label{fig:mqtt_latency}
% %     \vspace{-2ex}
% % \end{figure}

% \begin{figure}[htbp]
%     \centering
%     \subfloat []{\includegraphics[width=0.163\textwidth]{sections/Images/Mqtt_latency_new.png}}
%     \hfill
%     \subfloat []{\includegraphics[width=0.155\textwidth]{sections/Images/Mqtt_latency2_new.png}}
%     \hfill
%     \subfloat []{\includegraphics[width=0.162\textwidth]{sections/Images/differnt_distance_latency.png}}
%     % \vspace{-1ex}
%     \caption{MQTT latency for (a) different network bands \& image sizes,  (b) different split ratios, \& (c) different distances with differing velocities of UGVs}
%     \label{fig:mqtt_latency}
%     % \vspace{-2ex}
% \end{figure}


% Considering latency minimization we use 5GHz WiFi network bands in our work.
% In our study, we tested 100 images using the MQTT protocol for offloading images from the primary to the auxiliary node to run our multi-DNN model and evaluated the performance at different split ratios. Fig. \ref{fig:mqtt_latency}(b)  represents our outcomes.
% % \begin{figure}[htbp]
% %     % \vspace{-5ex}
% %     \centering
% %     \includegraphics[width=.20\textwidth]{sections/Images/Mqtt_latency2.png}
% %     \hfill
% %     \caption{For different network bands \& different sizes of images latency for MQTT protocol are different. It will change with the size of the images }
% %     \label{fig:mqtt_latency2}
% %     \vspace{-2ex}
% % \end{figure}
% In that case, latency is increasing with more offloading. For the 5 GHz bands and 50 KB images, 100\% offloading takes on average 9.32 ms per image. On the other hand, for 2.4 GHz it takes 21.15 ms per image. By using the 5 GHz bands, we are able to minimize huge latency. In addition, we measure offloading latency with varying distances of UGVs as shown in Fig. \ref{fig:mqtt_latency} (c) which depicts the increase in latency with distance. 
% %offloading latency with different distance
% % \begin{figure}[htbp]
% %     % \vspace{-5ex}
% %     \centering
% %     \includegraphics[width=.25\textwidth]{sections/Images/differnt_distance_latency.png}
% %     \hfill
% %     \caption{Recorded MQTT latency for different distances (UGVs have different velocity) }
% %     \label{fig:differnt_velocity}
% %     \vspace{-2ex}
% % \end{figure}

% \subsection{Device Profiling}

% % In our evaluation of the multi-DNN execution system, we profiled the primary and auxiliary nodes to measure their performance. The Jetson Nano served as the primary node, while the Jetson Xavier acted as the auxiliary. Both of them are resource-constraint devices. We aimed to offload images from the master to the slave when the latter had more processing power to spare. To determine the system's performance, we measured the memory utilization, power consumption, and inference time of both devices.

% % For memory utilization, we used the ‘free’ command-line utility to measure the memory usage of each device. The results indicated that the slave had a higher memory utilization compared to the master, due to its larger memory size. Nevertheless, the master node demonstrated efficient memory management with minimal memory fragmentation.

% % Power consumption was measured using Jetson stats. The results showed that the Jetson Xavier had a higher power consumption compared to the Jetson Nano. This is due to its higher processing power and memory size.

% % In terms of the operation time, we recorded the time taken for each device to perform image processing tasks. The results showed that the slave had a faster operation time compared to the master.
% % Following the execution of these two models on both devices, we have produced our initial baseline which is represented in Table \ref{tab:profile_table}. keeping track of the CPU and GPU utilization, as well as the percentage of memory usage and the operation time.

% % In our multi-DNN execution system, we utilized the multiprocessing pool to run semantic segmentation and posture detection simultaneously. The multiprocessing pool allowed us to take advantage of the parallel processing capabilities of the master and slave devices. 

% % Initially, we have 100 images to offload. Based on the master's capability and free memory and power usage, we increase the image offloading task to 0\% to 100\% and recorded all values for both devices  which are represented in Table \ref{tab:profile_table}.

% In our evaluation of the multi-DNN execution system, we profiled the Jetson Nano as the primary node and Jetson Xavier as the auxiliary node. We aimed to offload images when the auxiliary node had more processing power available. We measured memory utilization, power consumption, and inference time for both devices. The results showed higher memory utilization for the auxiliary node due to its larger memory size, while the primary node demonstrated efficient memory management with minimal fragmentation.

% We measure power consumption using Jetson stats, showing Jetson Xavier consumes more power than Jetson Nano due to higher processing power and memory size. We also record operation times for image processing tasks, with the auxiliary being faster than the primary node (Table \ref{tab:profile_table}).

% We use multiprocessing pool in our multi-DNN system to run semantic segmentation and posture detection concurrently, leveraging the parallel processing capabilities of primary and auxiliary devices.

% We start with 100 images to offload and adjust the offloading task from 0\% to 100\% based on the primary node's capacity, free memory, and power usage. The resulting values for both devices are recorded in Table \ref{tab:profile_table}.

% In our work, we propose the split ratio, which represents the proportion of images offloaded to the auxiliary node. This is an important parameter that can affect both the performance of the system and the resource utilization on both devices. It ranges from 0\% (all images processed locally) to 100\% (all images offloaded to the auxiliary). The optimal split ratio maximizes system performance while minimizing resource consumption. Notations $T1$, $P1$, and $M1$ represent operation time, power, and memory usage of the slave, while $T2$, $P2$, and $M2$ represent those of the primary node.

% % In our work, we propose a term split ratio, which refers to the proportion of images that are offloaded to the more powerful device (in this case, the slave). When we split our data into two portions, one is processed locally on the master while the other is offloaded to the slave for processing. The split ratio is the percentage of images that are offloaded to the agent device and can range from 0\% (all images handled locally) to 100\%  (all images offloaded to the slave). This is an important parameter that can affect both the performance of the system and the resource utilization on both devices. By determining the optimal split ratio, we may maximize overall system performance while minimizing resource consumption.
% % Here we showed some important points of split ratio r which is mainly how many images are split. Here $T1$, $P1$, and $M1$ indicate the total operation time, power, and memory usage of the slave. $T2$, $P2$, and $M2$ indicate the total operation time, power, and memory usage of the master. 


% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% % \usepackage[table,xcdraw]{xcolor}
% % If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


% % \begin{table}[htbp]
% % \centering
% % \Huge
% % \caption{Profiling results from testbed  for semantic segmentation and posture estimation model}
% % \label{tab:profile_table}
% % \setlength{\tabcolsep}{4pt}
% % \renewcommand{\arraystretch}{1.8}
% % \resizebox{1\linewidth}{!}{%
% % % \resizebox{\columnwidth}{!}{%
% % \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
% % \hline
% % {\color[HTML]{000000} \textbf{r (split ratio)}} &
% %   {\color[HTML]{000000} \textbf{$\mathrm{T_{1}}$ (Xavier) (s)}} &
% %   {\color[HTML]{000000} \textbf{$\mathrm{P_{1}}$ (Xavier)(w)}} &
% %   {\color[HTML]{000000} \textbf{$\mathrm{M_{1}}$ (Xavier)(\%)}} &
% %   {\color[HTML]{000000} \textbf{1-r}} &
% %   {\color[HTML]{000000} \textbf{$\mathrm{T_{2}}$ (Nano)(s)}} &
% %   {\color[HTML]{000000} \textbf{$\mathrm{T_{3}}$ (latency) (s)}} &
% %   \textbf{$\mathrm{P_{2}}$ (nano) (w)} &
% %   \textbf{$\mathrm{M_{2}}$ (nano)(\%)} \\ \hline
% % 0   & 0      & 0    & 0     & 1   & 68.34 & 0    & 5.89 & 69.82 \\ \hline
% % 0.3 & 8.45   & 4.59 & 36.67 & 0.7 & 39.03 & 0.43 & 5.35 & 63.77 \\ \hline
% % 0.5 & 13.88  & 5.42 & 45.61 & 0.5 & 28.35 & 0.89 & 5.63 & 52.54 \\ \hline
% % 0.7 & 16.64  & 5.73 & 51.23 & 0.3 & 19.54 & 1.25 & 4.75 & 45.58 \\ \hline
% % 0.8 & 17.24  & 6.17 & 56.96 & 0.2 & 13.34 & 1.44 & 4.48 & 40.34 \\ \hline
% % 1   & 19.001 & 6.38 & 59.37 & 0   & 0     & 1.56 & 0    & 0     \\ \hline
% % \end{tabular}
% % }
% % \end{table}
% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% % \usepackage[table,xcdraw]{xcolor}
% % If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

% \begin{table}[htbp]
% \centering
% \caption{Profiling results from testbed for semantic segmentation and posture estimation model}
% \label{tab:profile_table}
% \setlength{\tabcolsep}{4pt}
% \renewcommand{\arraystretch}{1.2}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
% \hline
% {\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}}r \\ (split ratio)\end{tabular}}} &
%   {\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}} \textbf{$T_{1}$} \\ (Xavier) \\ (s)\end{tabular}}} &
%   {\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}} \textbf{$P_{1}$} \\ (Xavier)\\ (w)\end{tabular}}} &
%   {\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}} \textbf{$M_{1}$} \\  (Xavier)\\ (\%)\end{tabular}}} &
%   {\color[HTML]{000000} \textbf{1-r}} &
%   {\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}} \textbf{$T_{2}$} \\  (Nano)\\ (s)\end{tabular}}} &
%   {\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}} \textbf{$T_{3}$} \\ (Offloading latency)\\  (s)\end{tabular}}} &
%   {\color[HTML]{000000} \textbf{\begin{tabular}[c]{@{}c@{}} \textbf{$P_{2}$} \\ (nano) \\ (w)\end{tabular}}} &
%   \textbf{\begin{tabular}[c]{@{}c@{}} \textbf{$M_{2}$} \\ (nano)\\ (\%)\end{tabular}} \\ \hline
% {\color[HTML]{000000} 0} &
%   {\color[HTML]{000000} 0} &
%   {\color[HTML]{000000} 0} &
%   {\color[HTML]{000000} 0} &
%   {\color[HTML]{000000} 1} &
%   {\color[HTML]{000000} 68.34} &
%   {\color[HTML]{000000} 0} &
%   {\color[HTML]{000000} 5.89} &
%   {\color[HTML]{000000} 69.82} \\ \hline
% {\color[HTML]{000000} 0.3} &
%   {\color[HTML]{000000} 8.45} &
%   {\color[HTML]{000000} 4.59} &
%   {\color[HTML]{000000} 36.67} &
%   {\color[HTML]{000000} 0.7} &
%   {\color[HTML]{000000} 39.03} &
%   {\color[HTML]{000000} 0.43} &
%   {\color[HTML]{000000} 5.35} &
%   {\color[HTML]{000000} 63.77} \\ \hline
% {\color[HTML]{000000} 0.5} &
%   {\color[HTML]{000000} 13.88} &
%   {\color[HTML]{000000} 5.42} &
%   {\color[HTML]{000000} 45.61} &
%   {\color[HTML]{000000} 0.5} &
%   {\color[HTML]{000000} 28.35} &
%   {\color[HTML]{000000} 0.89} &
%   {\color[HTML]{000000} 5.63} &
%   {\color[HTML]{000000} 52.54} \\ \hline
% {\color[HTML]{000000} 0.7} &
%   {\color[HTML]{000000} 16.64} &
%   {\color[HTML]{000000} 5.73} &
%   {\color[HTML]{000000} 51.23} &
%   {\color[HTML]{000000} 0.3} &
%   {\color[HTML]{000000} 19.54} &
%   {\color[HTML]{000000} 1.25} &
%   {\color[HTML]{000000} 4.75} &
%   {\color[HTML]{000000} 45.58} \\ \hline
% {\color[HTML]{000000} 0.8} &
%   {\color[HTML]{000000} 17.24} &
%   {\color[HTML]{000000} 6.17} &
%   {\color[HTML]{000000} 56.96} &
%   {\color[HTML]{000000} 0.2} &
%   {\color[HTML]{000000} 13.34} &
%   {\color[HTML]{000000} 1.44} &
%   {\color[HTML]{000000} 4.48} &
%   {\color[HTML]{000000} 40.34} \\ \hline
% {\color[HTML]{000000} 1} &
%   {\color[HTML]{000000} 19.001} &
%   {\color[HTML]{000000} 6.38} &
%   {\color[HTML]{000000} 59.37} &
%   {\color[HTML]{000000} 0} &
%   {\color[HTML]{000000} 0} &
%   {\color[HTML]{000000} 1.56} &
%   {\color[HTML]{000000} 0} &
%   {\color[HTML]{000000} 0} \\ \hline
% \end{tabular}%
% }
% \end{table}


% Overall, the profiling results indicated that the auxiliary node is a more powerful device compared to the primary node. However, the primary node demonstrated efficient resource management and was able to effectively offload tasks to the auxiliary node when needed. These results highlight the benefits of using a multi-DNN execution system, as it allows for efficient utilization of resources and faster processing times. By using multiple processors, we were able to run multiple DNN models at the same time, resulting in a significant reduction in processing time.
% \begin{figure}[http]
%     % \vspace{-5ex}
%     \centering
%     \includegraphics[width=.5\textwidth]{sections/Images/profiling_results_new.png}
%     \hfill
%     \caption{Profiling results from testbed, a) Time taken by both devices at different split ratios. b)Total time and memory usage for different split ratios. c) Power usage for both devices (d) Recorded MQTT latency and inference time for different split ratios}
%     \label{fig:profiling_results}
%     % \vspace{-2ex}
% \end{figure}
% The profiling results show that running the model on a single device (nano) takes nearly 69.82 seconds for total operation( loading model, Image sending time, and Inference time)  and to process 100 images for both models combined.  This resulted in high utilization of memory and power, causing the device to become overloaded. To alleviate this issue, we decided to offload some of the images to a more powerful device, the Jetson Xavier. By doing so, we were able to significantly reduce the inference time and minimize the utilization of memory and power. From Fig. \ref{fig:profiling_results} (d) we see the changes in inference time with respect to a higher split ratio.

% \begin{figure}[htbp]
%     % \vspace{-5ex}
%     \centering
%     \includegraphics[width=.20\textwidth]{sections/Images/Mqtt_inference_bar_new.png}
%     \hfill
%     \caption{Recorded MQTT latency and inference time for different split ratio }
%     \label{fig:mqtt_Inference}
%     \vspace{-2ex}
% \end{figure}



% To begin, we created a fundamental baseline before beginning the investigations. On edge devices, we have implemented the Yolov5 object detection model in conjunction with the semantic segmentation model. We made the decision to run each model independently on the Raspberry pi 4B and the Jetson nano and to keep track of their CPU, GPU, and memory utilization as well as their inference time. The Jetson Nano contains a GPU, in contrast to the Raspberry Pi 4B, which does not.

% The system-on-a-chip (SoC) used in the Raspberry Pi 4B is a Broadcom BCM2711, which features a 1.5 GHz, 64-bit quad-core ARM Cortex-A72 processor (four-core CPU). A compact and potent personal computer, the Jetson Nano features a quad-core ARM Cortex-A57 MPCore processor (four core CPU), an integrated 128-core Maxwell GPU, and 4 gigabytes of LPDDR4 memory. When set next to one another, the Jetson Nano possesses a great deal more computational capability than the Raspberry Pi 4B.\\

% It is not simple to use this device, which has limited resources, to run a deep learning model. We have no choice but to work with a model that is capable of accommodating edge devices such as the Raspberry Pi and the Jetson Nano. One of the difficulties was posed by this. We have employed the YoloV5 model, which is composed of the following three components: (1) CSPDarknet serves as the backbone of the network, (2) PANet serves as the neck, and (3) Yolo Layer serves as the head. The data are initially supplied into CSPDarknet for the purpose of feature extraction, and then they are transferred to PANet for the purpose of feature fusion. At the end of the process, Yolo Layer will output detection results (class, score, position, and size)\cite{Yolov5}.\\


% As a result of the findings, we came to the conclusion that the Jetson nano possesses a higher level of computational capability than the Raspberry pi 4B. When calculating Yolov5 tiny weights, the inference time required by the Jetson nano was 0.18 seconds, while the time required by the Raspberry Pi 4B was 0.967 seconds. In the case of middling weights, it took 0.41 seconds for the Jetson nano to complete the task, whereas it took 2.1 seconds for the Raspberry Pi 4B.\\
% On every given device, we can only run a single deep-learning model at a time. The Yolov5 model itself consumes fifty percent of the processing power available to the Raspberry Pi 4B. It utilized over half of the graphics processing unit (GPU) of more capable Jetson devices and a sizeable portion of the central processing unit (CPU). In essence, it is to support the primary problem statements that we have. The use of multiple deep learning models in parallel on devices with limited resources necessitates optimization and the implementation of an appropriate code offloading architecture. The technique that we have proposed makes it possible to execute multiple programs concurrently on devices with limited resources.

% \section{\textbf{Optimization Framework}}
% We have designed a memory- and power-aware multi-DNN optimization framework (Fig. \ref{fig:framework}) for edge devices. The framework enables efficient image offloading to auxiliary node and DNN model processing on both devices with split images. Our optimization framework can achieve the lowest inference time for both devices at a given data-splitting ratio while ensuring that both devices have enough memory and power. The framework dynamically adjusts the data splitting ratio based on the available resources on the primary node and the auxiliary. When the master node lacks the memory or power to process the models at a specific ratio, the framework offloads some data to the more powerful agent to ensure efficient processing. This optimization framework provides a solution for optimizing multi-DNN application performance and resource utilization on edge devices.

% Our optimization approach provides a cost-effective solution for edge computing in addition to the efficient processing of multi-DNN models. By utilizing the resources of both the master node and the agent, the framework minimizes the waste of resources and reduces the energy consumption of the system. This is particularly important in edge computing, where devices have limited resources and energy constraints. Our framework can be applied to various edge computing scenarios and easily adapt to changing requirements and environments. The framework is also scalable and can be applied to systems with multiple edge devices, enabling the efficient processing of large amounts of data in a distributed manner. Overall, our memory- and power-aware multi-DNN optimization framework offers a dependable and efficient solution for edge computing applications.
% \begin{figure}[htbp]
%     \centering
%     \includegraphics[scale = 0.18]{sections/Images/Optimization_pipeline.png}
%     \hfill
%     \caption{ Optimization framework overview}
%     \label{fig:framework}
% \end{figure}



% \begin{figure}[htbp]
%     \centering
%     \subfloat []
%     {\includegraphics[width=0.28\textwidth]{sections/Images/framework1.png}}
%     \hfill
%     \subfloat []
%     {\includegraphics[width=0.20\textwidth]{sections/Images/framework2.png}}
%     % \vspace{-1ex}
%     \caption{Optimization framework overview: (a) Frame compression technique (b) Task scheduling process }
%     \label{fig:framework}
%     % \vspace{-2ex}
% \end{figure}









==> sections/Introduction.tex <==
\section{\textbf{Introduction}}
Unmanned aerial vehicles (UAVs) or drones have recently become popular for various societal applications such as search and rescue operations, disaster monitoring and damage assessment etc. They can be easily deployed and controlled to provide various critical and just-in-time information for events which are often inaccessible to humans.
%They manifest in a wide variety of uses for economic, commercial, recreational, military, and academic purposes. 
Despite these tempting advantages, UAVs have limited functioning due to a number of important constraints about flight time and battery capacity\cite{2023mohsanspringer}.
Flight time is a crucial aspect of unmanned aerial vehicles (UAVs), as it directly impacts their operational capabilities\cite{2022droneflight}. One of the major limitations faced by UAVs is the limited power supply, which results in reduced flight time\cite{2019hashemi}. This problem is exacerbated by the increasing power consumption requirements of various onboard systems, such as navigation systems, cameras, and communication systems\cite{2021khochare}.
Running a deep neural network (DNN) application on a drone during flight can have a significant impact on both flight time and power consumption. DNNs are computationally intensive, requiring significant processing power and energy consumption\cite{Heimdel}, which can shorten the flight time of the drone.

However, the effect on flight time and power consumption will depend on several factors, including the complexity of the DNN, the size of the data being processed, and the efficiency of the hardware and software used. Offloading some of the inference tasks to a remote device or UGV can have a positive impact on the power consumption of the drone. UAVs that developed using edge computing technology, scheduling edge computing tasks that are computed- and energy-aware, operating on distributed edge resources and considering memory and device reliability in consideration\cite{Meng2019DedasOT}.

This approach allows the drone to offload some of its computationally intensive tasks to a more powerful device, such as a cloud server\cite{xing2022}, or local-edge-cloud collaborative environment\cite{xue2022}, thereby reducing the power consumption and computational load. However, one of the major drawbacks of offloading tasks to remote servers is the potential for increased network latency. Network latency can arise due to the distance between the drone and the cloud server, as well as the quality of the communication link. Latency can impact the performance of the system, as well as the accuracy of the results. Offloading tasks to cloud servers also increases the dependence on the availability of the remote server. Offloading tasks to cloud servers often requires the use of cloud computing services, which can be costly, especially for large-scale deployments. Some IoE applications, such as face recognition, ultra-high-definition video, augmented reality (AR), virtual reality (VR), and semantic segmentation, require low latency and high processing performance, posing a challenge to traditional clouds' flexible and scalable computing models \cite{chen2022}.

In this paper, we offer an improved optimized tasks scheduling framework for multi-DNN applications from edge to edge that is very responsive and efficient for resource constraint devices. In the first place, we are going to employ two different applications: semantic segmentation, and posture recognition. In this scenario, we feed the system image data, which could be a raw image or a compressed image. The framework makes use of a scheduling architecture and resource allocation, while a Jetson nano, which possesses a less amount of computational capacity, operates as a master. Second, we run multiple applications on a master node, and that node is responsible for distributing DNN tasks to the other node Jetson Xavier which is more computationally powerful. The master node acts as a scheduler and divides up the offloading tasks to be completed among the free workers. We used the MQTT protocol to transfer images from master to agent using the publisher-subscriber system.
% Deep neural networks (DNNs) have demonstrated great potential for use in a variety of Internet of Things (IoT) and cyber-physical Systems (CPS) applications, such as autonomous driving\cite{Bojarski2016EndTE}\cite{csp} intelligent robotics\cite{Dyrstad2017GraspingVF} and military reconnaissance. New devices and technical concepts may be implemented in the military to increase and improve current resources. Multiple deep learning algorithms, such as object detection, face recognition, and image segmentation, can be implemented in military settings to improve intelligence and surveillance. In such systems, raw sensor data is collected by multiple sensing tasks, which then send DNN inference requests (jobs) to different pre-trained DNN models in order to get a high-level representation of the environment.\\
% Unfortunately, current cutting-edge deep learning frameworks, such as TensorFlow and PyTorch, are not well suited to serving multiple applications on edge devices because they were designed and optimized to execute a single DNN as quickly as possible. They handle inference jobs sequentially, with a single process for each DNN model. When dealing with batch jobs, this method is useful for achieving high throughput. When serving multiple inference requests, they miss out on opportunities to use all processors. Multiple DNNs can technically run on a single processor, but devices like the Jetson Nano and Raspberry Pi are too resource-constrained to serve multiple inference tasks. Multi-core CPUs and hardware accelerators like GPUs have been used to improve the average response time of inference jobs. However, when multiple DNN models are requested at the same time, they are often not used to their full potential, and their benefits in the worst case are not as great as in the average case.\\
% The execution of the CNN's convolution layers requires a lot of CPU and GPU power, whereas the computing of the CNN's fully-connected layers requires a lot of memory due to the large number of weights used in the model. Our framework currently supports four ARM Cortex-A72 CPU cores of the Raspberry pi 4B, four ARM Cortex-A57 CPUs of the Jetson nano, and one Nvidia-integrated 128-core Maxwell GPU of the Jetson nano. You have two Raspberry Pi 4B and one Jetson nano, which are connected to each other as nodes.\\
 %Each model was subdivided into several smaller models. Smaller models have been split by layer from the mother model, and their weight parameters are stored in a separate file. 

% Current state-of-the-art mobile deep learning frameworks are not capable of handling multiple deep learning algorithms concurrently. There exist GPU constraints where contention of multiple deep neural networks, or DNNs, slows down inference latency immensely\cite{Heimdel}. This is a problem if we want to deploy
% wireless sensor networks into real applications, as we would need the network to run in real-time. Mobile processors and edge devices, such as Jetson Nanos and Raspberry Pis are extremely limited in their resources and computational power. Due to limited architectural support and memory bandwidth,
% this will be another concern that we must take into consideration while studying the organization of wireless sensor networks and how we may optimize it.\\
% We want to run several deep learning applications concurrently on an asymmetric wireless sensor network, and in order to do so, we study the organization of a smaller wireless sensor network simulation. We aim for high accuracy in the execution of the concurrent deep learning algorithms, as well as low bandwidth among the asymmetric wireless sensor network.\\
In contrast, our contributions in this paper are as follows:
\begin{itemize}
\item \textbf{Resource-aware novel offloading algorithm for latency minimization}          
We propose a resource-aware novel offloading algorithm for latency minimization specifically for edge devices. This algorithm takes into account the limited resources (such as processing power, memory, and network bandwidth) of these devices and uses this information to determine the best location (local device) to execute a task, in order to reduce latency and optimize performance. The goal of this type of offloading algorithm is to minimize latency for edge devices, which are often required to respond to real-time events. 
\item \textbf{Data-driven derivation of optimization constraints through profiling on heterogeneous systems}       
We derive the constraints used to form the optimization framework through heterogeneous device profiling to determine the trend of resource consumption for multi-DNN applications. The goal of this type of resource profiling is to obtain a comprehensive understanding of the resources available at the edge devices, which can then be used to optimize the performance of applications and services running on these devices. By using heterogeneous off-the-shelf edge devices, we profile the important available resources like processing power, memory, and total operation times, which include image transfer time from one device to another, model loading time, and inference time. This helps us determine how efficiently we distribute workloads from master to agents.
\item \textbf{Customized testbed design and empirical evaluation on datasets of different modalities}
We have designed a WSN testbed for our experimentation scenario, integrated with a customized MQTT-based publisher-subscriber protocol. Furthermore, in order to validate the ubiquitous adaptation of our proposed optimization framework, we evaluate its performance on applications with various data modalities. We have achieved similar results on applications like poster detection, semantic segmentation, and object detection for relevant evaluating matrices.
 
\end{itemize}

